Protecting real-time GPU kernels on integrated CPU-GPU SoC platforms

Integrated CPU-GPU architecture provides excellent acceleration capabilities for data parallel applications on embedded platforms while meeting the size, weight and power (SWaP) requirements. However, sharing of main memory between CPU applications and GPU kernels can severely affect the execution of GPU kernels and diminish the performance gain provided by GPU. For example, in the NVIDIA Tegra K1 platform which has the integrated CPU-GPU architecture, we noticed that in the worst case scenario, the GPU kernels can suffer as much as 4X slowdown in the presence of co-running memory intensive CPU applications compared to their solo execution. In this paper, we propose a software mechanism, which we call BWLOCK++, to protect the performance of GPU kernels from co-scheduled memory intensive CPU applications.

==> sections/figures/fig-tt-throttling.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.32\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/CFS/tt_cfs-cropped.pdf}
	\caption{System Throttle Time with normal Throttling}
	\label{fig:tt-thrt}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/CFS/tt_tfs-cropped.pdf}
	\caption{System Throttle Time with TFS}
	\label{fig:tt-tfs}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
	\centering
	\includegraphics[width=\textwidth]{figures/CFS/tt_tfs3-cropped.pdf}
	\caption{System Throttle Time with TFS-3X}
	\label{fig:tt-tfs3}
\end{subfigure}
\caption{System throttle time progression under different throttling schemes}
\label{fig:tt-throttling}
\end{figure}


==> sections/tables/tbl-benchmarks.tex <==
\begin{table}[h]
	\centering
		\begin{tabularx}{\linewidth}{ p{1.5cm} | p{2.3cm} | p{8.9cm}}
		\toprule
		Benchmark 	 & Dataset & Description \\
		\midrule
		histo		 & Large   	   & Computation of 2-D saturating histogram \\
		sad		 & Large	   & Sum of absolute differences benchmark used in motion estimation \\
		bfs		 & 1-Million Nodes & Graph based breadth first search algorithm \\
		spmv		 & Large	   & Implementation of sparse matrix dense vector algorithm \\
		stencil		 & Default 	   & An iterative Jacobi stencil operation on a regular 3-D grid \\
		lbm		 & Long   	   & Fluid dynamics simulation of an enclosed lid-driven cavity using the Lattice-Boltzmann method \\
		\bottomrule
		\end{tabularx}
	\caption{Description of GPU benchmarks selected for BWLOCK++ evaluation}
	\label{tbl:benchmarks}
\end{table}


==> sections/tables/tbl-overhead.tex <==
\begin{table}[t]
	\centering
		\begin{tabular}{p{2.5cm} | p{2.5cm}}
		\toprule
		Benchmark & Overhead (\%) \\
		\hline
		histo & 0.618\\
		lbm & 0.195\\
		bfs & 0.588\\
		sad & 2.571\\
		stencil & 2.757\\
		spmv & 0.788\\
		\bottomrule
		\end{tabular}
	\caption{BWLOCK++ Overhead}
	\label{tbl:overhead}
\end{table}

